DiffTraj: Generating GPS Trajectory with Diffusion Probabilistic Model

Pervasive integration of GPS-enabled devices and data acquisition technologies has led to an exponential increase in GPS trajectory data, fostering advancements in spatial-temporal data mining research. Nonetheless, GPS trajectories contain personal geolocation information, rendering serious privacy concerns when working with raw data. A promising approach to address this issue is trajectory generation, which involves replacing original data with generated, privacy-free alternatives. Despite the potential of trajectory generation, the complex nature of human behavior and its inherent stochastic characteristics pose challenges in generating high-quality trajectories. In this work, we propose a spatial-temporal diffusion probabilistic model for trajectory generation (DiffTraj). This model effectively combines the generative abilities of diffusion models with the spatial-temporal features derived from real trajectories. The core idea is to reconstruct and synthesize geographic trajectories from white noise through a reverse trajectory denoising process. Furthermore, we propose a Trajectory UNet (Traj-UNet) deep neural network to embed conditional information and accurately estimate noise levels during the reverse process. Experiments on two real-world datasets show that DiffTraj can be intuitively applied to generate high-fidelity trajectories while retaining the original distributions. Moreover, the generated results can support downstream trajectory analysis tasks and significantly outperform other methods in terms of geo-distribution evaluations.

==> 04-Methodologyback.tex <==


% Clearly articulate the novelty of your research and its contributions to the field. Your paper should demonstrate how DiffTraj and the Trajectory UNet (Traj-UNet) address the challenges in generating high-quality trajectories and offer improvements over existing methods.
% Introduce the Traj-UNet deep neural network as a method to embed conditional information and estimate noise levels during the reverse process.
% Explain how Traj-UNet complements and enhances the DiffTraj model.

\section{Methodology}\label{sec:method}
In this section, we elaborate on the proposed Diff-Traj.
We start by presenting the fundamentals of the diffusion model, including two main processes, objective optimization function, and sampling speed-up methods.
Then, we introduce the details of the denoising model, i.e., Traj-UNet.





\subsection{DiffTraj Framework}\label{sec:diffModel}
% We first briefly introduce the theory of diffusion model (See literature \cite{ddpm} for more details).
As shown in \cref{fig:framework},  the Diff-Traj framework involves two main processes, namely, the forward trajectory noising process and the reverse trajectory denoising process.
The former aims to iteratively add noise to the trajectory sequence that ultimately converges into a Gaussian distribution.
The latter subsequently reconstructs the Gaussian noise for each step and eventually generates the GPS trajectory sequence \cite{ddpm,ddim,diffusionsuvery}.
At each step in the reverse trajectory denoising process, the noise is predicted by a designed neural network called Traj-UNet.

% As depicted in \cref{fig:framework},  the Diff-Traj framework involves two main processes, namely, the forward trajectory noising process and the reverse trajectory denoising process.
% For the forward trajectory noising process, the objective is to iteratively add noise to the trajectory sequence that ultimately converges into a Gaussian distribution.
% For the reverse trajectory denoising process, it restores the Gaussian noise for each step and eventually generates the GPS trajectory sequence.
% At each step in the denoising process, the noise is predicted by a designed neural network called Trajectory UNet.


% \note[02-02]{}{最好在这段概念性地描述一下你这个framework中的这两部分究竟是干啥的，目的是什么，如何实现的。}

% \subsubsection{Reparameterization}\label{sec:repar}



% \note[02-02]{which transforms the sampling results into a specific distribution,}{这个解释不够。读者不了解的话并不知道你要sample个什么东西，为什么需要转换成distribution} \note[02-02]{allowing for the derivation of the transformation process}{需要想一下如何从diffusion引入reparameterization}.
% Specifically, sampling $\boldsymbol{z} \sim \mathcal{N}\left(\boldsymbol{z} ; \boldsymbol{\mu}, \sigma^2 \mathbf{I}\right)$ from the standard Gaussian distribution can be formulated as:
% \begin{equation}\label{eq:trick}
%     \boldsymbol{z} = \boldsymbol{\mu}_{\theta} + \sigma_{\theta} \odot \boldsymbol{\epsilon}, \quad \boldsymbol{\epsilon} \sim \mathcal{N}(0, \mathbf{I}),
% \end{equation}
% where $\odot$ indicates element-wise product.
% According to this formula, $\boldsymbol{z} $ \note[02-02]{retains its randomness and satisfies a Gaussian distribution}{直接强调reparameterization的作用之一是让Gaussian sample可微} with mean $\boldsymbol{\mu}_{\theta}$ and variance $\sigma^2_{\theta}$.
% Here, $\boldsymbol{\mu}_{\theta}$ and $\sigma^2_{\theta}$ can be inferred from a parameterised neural network. 
% The entire sampling process remains gradient-derivative and the added randomness follows Gaussian $\boldsymbol{\epsilon}$.



\subsubsection{Forward Trajectory Noising Process}\label{sec:noising}
This process involves introducing noise to the initial trajectory while simultaneously learning its spatial-temporal features.
Since noise is stochastically created, it requires careful tuning to make sure that the resulting trajectories are realistic and free of any irrational behavior.
Additionally, this process requires an incremental approach to prevent excessive noise from severely biasing the trajectory or impairing the precision of its creation.
% \zxy{what is the challenges of this process? Otherwise, our contribution seems trivial}

% \zxy{to address above challenges...} 
To address above challenges, the forward process can be considered as step-wise noisifying the trajectory. 
Given a real-world trajectory sample $\boldsymbol{x} \sim q\left(\boldsymbol{x}\right)$, the forward process adds $T$ time-steps of Gaussian noise to it, where $T$ is an adjustable parameter.
Subsequently, each step holds a noise trajectory and obtains a set of noisy trajectories $\left\{\boldsymbol{x}_{0}, \boldsymbol{x}_{1}, \ldots, \boldsymbol{x}_{T} \right\}$.
In practice, we consider the $\boldsymbol{x}_0$ indicates the raw trajectory without any manipulation.
$\boldsymbol{x}_t$ loses its spatial-temporal features as $t$ increases and finally converges into a unit Gaussian $\boldsymbol{x}_{T} \sim \mathcal{N}\left(0, \mathbf{I} \right)$.
Since it is a step-by-step chain calculation, we can express it as a Markov process:
% cumulatively to obtain \fix{the noisy trajectory sequences}{a set of noisy trajectories} $\left\{\boldsymbol{x}_{0}, \boldsymbol{x}_{1}, \ldots, \note[02-02]{\boldsymbol{x}_{T}}{大T是怎么设置的？与原始traj的点数相同？}\right\}$.
% \note[02-02]{(the subscript $0$ indicates a real trajectory without any manipulation)}{这种标号很奇怪to me。可以考虑原始的用黑x，生成的用tilde黑x，后者从0开始index}.
% The forward process adds $T$ time\fix{ }{-}steps \fix{}{of }Gaussian noise\notemar[02-02]{读完这小段，我觉得这个地方可能有问题。读者会很懵为什么要加T步的噪音，这个操作的intuition和目的是什么？ 在第一段添加了描述} to \fix{real trajectory}{} $\boldsymbol{x}_{0}$ cumulatively to obtain \fix{the noisy trajectory sequences}{a set of noisy trajectories} $\left\{\boldsymbol{x}_{0}, \boldsymbol{x}_{1}, \ldots, \note[02-02]{\boldsymbol{x}_{T}}{大T是怎么设置的？与原始traj的点数相同？}\right\}$.
% Since each step $t$ in this process \note[02-02]{depends on}{英文语境中，step不会depend on step。是step中的计算depends。chaining calculation} step $t-1$, it can also be expressed as a Markov process:
\begin{equation}\label{eq:forward}
\begin{aligned}
    q\left(\boldsymbol{x}_t \mid \boldsymbol{x}_{t-1}\right)&=\mathcal{N}\left(\boldsymbol{x}_t ; \sqrt{1-\beta_t} \boldsymbol{x}_{t-1}, \beta_t \mathbf{I}\right)\\
    q\left(\boldsymbol{x}_{1: T} \mid \boldsymbol{x}_0\right)&=\prod_{t=1}^T q\left(\boldsymbol{x}_t \mid \boldsymbol{x}_{t-1}\right),
\end{aligned}
\end{equation}
where $\mathcal{N}\left( \cdot \right)$ denotes Gaussian noise and $\{\beta_t \in (0,1)\}_{t=1}^{T}$ ($ \beta_1 < \beta_2 < \ldots < \beta_T$) is the corresponding variance schedule.
Let $\alpha_{t}=1-\beta_t$ and $\bar{\alpha}_t=\prod_{i=1}^{t}\alpha_i$. 
Since it is impractical to backpropagate the gradient by sampling from a Gaussian distribution, we adopt a reparameterization trick to keep the gradient derivable \cite{ddpm}.
Specifically, sampling $\boldsymbol{z} \sim \mathcal{N}\left(\boldsymbol{z} ; \boldsymbol{\mu}, \sigma^2 \mathbf{I}\right)$ from the standard Gaussian distribution can be formulated as:
\begin{equation}\label{eq:trick}
    \boldsymbol{z} = \boldsymbol{\mu}_{\theta} + \sigma_{\theta} \odot \boldsymbol{\epsilon}, \quad \boldsymbol{\epsilon} \sim \mathcal{N}(0, \mathbf{I}),
\end{equation}
where $\odot$ indicates element-wise product.
% According to this formula, $\boldsymbol{z} $ \note[02-02]{retains its randomness and satisfies a Gaussian distribution}{直接强调reparameterization的作用之一是让Gaussian sample可微} with mean $\boldsymbol{\mu}_{\theta}$ and variance $\sigma^2_{\theta}$.
% Here, $\boldsymbol{\mu}_{\theta}$ and $\sigma^2_{\theta}$ can be inferred from a parameterised neural network. 
% The entire sampling process remains gradient-derivative and the added randomness follows Gaussian $\boldsymbol{\epsilon}$.
According to this trick, $\boldsymbol{x}_t$ can be written as:
\begin{equation}\label{eq:repara}
\begin{aligned}
\boldsymbol{x}_t&=\sqrt{\alpha_t} \boldsymbol{x}_{t-1}+\sqrt{1-\alpha_t} \boldsymbol{\epsilon}_{t-1} \\
&=\sqrt{\alpha_t \alpha_{t-1}} \boldsymbol{x}_{t-2}+\sqrt{1-\alpha_t \alpha_{t-1}} \overline{\boldsymbol{\epsilon}}_{t-2}  \\
& = \dots \\
& =\sqrt{\bar{\alpha}_t} \boldsymbol{x}_0+\sqrt{1-\bar{\alpha}_t} \boldsymbol{\epsilon} ,
\end{aligned}
\end{equation}
where $\epsilon_t \sim \mathcal{N}(0,\mathbf{I})$ and $\bar{\epsilon}_t$ is the aggregation of two Gaussian distributions.
Then, \cref{eq:forward} can be rewritten as:
\begin{equation}\label{eq:qxtx0}
     q\left(\boldsymbol{x}_t \mid \boldsymbol{x}_{0}\right)=\mathcal{N}\left(\boldsymbol{x}_t ; \sqrt{\bar{\alpha}_t} \boldsymbol{x}_{0}, (1-\bar{\alpha}_t) \mathbf{I}\right).
\end{equation}
As a result, we can sample from a Gaussian at any time step to obtain the noisy trajectory $\boldsymbol{x}_t$.
During this process, a tailored deep neural network is applied to learn the spatial-temporal characteristics of the corresponding noise level.

% During this process, real trajectory gradually \note[02-02]{loses its spatial-temporal features}{这对隐私保护是好事，但是听起来对特征提取是坏事。像个别的写法} as $t$ increases. 
% \note[02-02]{When $T \to \infty$, $\boldsymbol{x}_{T}$ converges into standard Gaussian noise $\mathcal{N}\left(0, \mathbf{I} \right)$.}{啥？}


\begin{figure*}[t]
	\centering
	\includegraphics[width=0.95\linewidth]{Figures/UNet1.pdf}
	\caption{The structure of Traj-UNet is divided into two modules, down-sampling and up-sampling, each of which contains multiple Resnet blocks. For each Resnet block, the time step and external attribute embedding are integrated.}
	\label{fig:structure}
\end{figure*}

\subsubsection{Reverse Trajectory Denoising Process}\label{sec:denoising}
This process takes Gaussian noise as the input and infers the forged trajectory.
During this process, the most challenging point is estimating the noise level from the noisy input trajectory. 

% This process  takes Gaussian noise $\boldsymbol{x}_{T} \sim \mathcal{N}\left(0, \mathbf{I} \right)$ as the input, aims to forge trajectories by a stepwise denoising process.
% After the forward trajectory noising process, the reverse denoising process takes Gaussian noise $\boldsymbol{x}_{T} \sim \mathcal{N}\left(0, \mathbf{I} \right)$ as the input, infers the noise\fix{}{,}\note[02-02]{}{三个或三个以上，全部有逗号。否则就变成I have two children, Alice and Bob.} and \note[02-02]{reconstructs the real trajectory}{读起来很奇怪。目标是重构真实轨迹的话，与隐私保护的目标冲突。我明白你的意思是过程中有perturbation，但是这样写就会有这种感觉。} $\boldsymbol{x}_{0}$.
% \zxy{what is the challenges of this process? Otherwise, our contribution seems trivial}
To tackle this challenge, in practice, we can implement the denoising process in a stepwise $\boldsymbol{x}_t \to \boldsymbol{x}_{t-1}$ manner.
Since estimating the reverse conditional probability $q\left(\boldsymbol{x}_{t-1} \mid \boldsymbol{x}_{t}\right)$ is intractable \cite{ddpm,ddim}, which can use a parameterized neural network $p_{\theta}$ to approximate this process:
\begin{equation}\label{eq:bprocess}
\begin{aligned}
p_\theta\left(\boldsymbol{x}_{t-1} \mid \boldsymbol{x}_t\right) & =\mathcal{N}\left(\boldsymbol{x}_{t-1} ; \mu_\theta\left(\boldsymbol{x}_t, t\right), \Sigma_\theta\left(\boldsymbol{x}_t, t\right)\right), \\
p_\theta\left(\boldsymbol{x}_{0: T}\right) & =p_\theta\left(\boldsymbol{x}_T\right) \prod_{t=1}^T p_\theta\left(\boldsymbol{x}_{t-1} \mid \boldsymbol{x}_t\right), 
% p_\theta\left(\boldsymbol{x}_0\right) & =\int p_\theta\left(\boldsymbol{x}_{0: T}\right) d \boldsymbol{x}_{1: T},
\end{aligned}
\end{equation}
where $\mu_\theta\left(x_t, t\right)$ and $\Sigma_\theta\left(x_t, t\right)$ are the mean and variance, respectively.
With the Bayesian formula, the reverse conditional probability can be derived when conditioned on $\boldsymbol{x}_0$:
\begin{equation}\label{eq:cond}
    q\left(\boldsymbol{x}_{t-1} \mid \boldsymbol{x}_t, \boldsymbol{x}_0\right)  =\mathcal{N}\left(\boldsymbol{x}_{t-1} ;\tilde{\mu}_t\left(\boldsymbol{x}_t, \boldsymbol{x}_0\right), \tilde{\beta}_t \mathbf{I}\right),
\end{equation}
where
\begin{equation}\label{eq:mubart}
\begin{aligned}
\tilde{\mu}_t\left(\boldsymbol{x}_t, \boldsymbol{x}_0\right) & =\frac{\sqrt{\bar{\alpha}_{t-1}} \beta_t}{1-\bar{\alpha}_t} \boldsymbol{x}_0+\frac{\sqrt{\alpha_t}\left(1-\bar{\alpha}_{t-1}\right)}{1-\bar{\alpha}_t} \boldsymbol{x}_t \\
\tilde{\beta}_t & =\frac{1-\bar{\alpha}_{t-1}}{1-\bar{\alpha}_t} \beta_t.
\end{aligned}
\end{equation}
Based on \cref{eq:repara}, replacing \cref{eq:mubart} with $\boldsymbol{x}_0=\frac{1}{\sqrt{\bar{\alpha}_t}}(\boldsymbol{x}_t - \sqrt{1-\bar{\alpha}_t} \boldsymbol{\epsilon})$, we have:
% \note[02-02]{substituting}{substitute something for the original thing}  
\begin{equation}\label{eq:mut}
\tilde{\boldsymbol{\mu}}_t =\frac{1}{\sqrt{\alpha_t}}\left(\boldsymbol{x}_t-\frac{1-\alpha_t}{\sqrt{1-\bar{\alpha}_t}} \boldsymbol{\epsilon}\right).
\end{equation}
% \begin{aligned}
% \tilde{\boldsymbol{\mu}}_t & =\frac{\sqrt{\alpha_t}\left(1-\bar{\alpha}_{t-1}\right)}{1-\bar{\alpha}_t} \boldsymbol{x}_t+\frac{\sqrt{\bar{\alpha}_{t-1}} \beta_t}{1-\bar{\alpha}_t} \frac{1}{\sqrt{\bar{\alpha}_t}}\left(\boldsymbol{x}_t-\sqrt{1-\bar{\alpha}_t} \boldsymbol{\epsilon}\right) \\
% & =\frac{1}{\sqrt{\alpha_t}}\left(\boldsymbol{x}_t-\frac{1-\alpha_t}{\sqrt{1-\bar{\alpha}_t}} \boldsymbol{\epsilon}\right).
% \end{aligned}
% \end{equation}
Here, the Gaussian distribution $\boldsymbol{\epsilon}$ is the noise predicted by the neural network model (for denoising), i.e., $\boldsymbol{\epsilon}_{\theta}(\boldsymbol{x}_t,t)$, which gives:
\begin{equation}\label{eq:mutheta}
\mu_\theta\left(x_t, t\right)=\frac{1}{\sqrt{\alpha_t}}\left(\boldsymbol{x}_t-\frac{\beta_t}{\sqrt{1-\bar{a}_t}} \epsilon_\theta\left(\boldsymbol{x}_t, t\right)\right).
\end{equation}
For convenience of calculation, $\Sigma_\theta\left(\boldsymbol{x}_t, t\right) = \sigma_t^2\mathbf{I}$ and $\sigma_t^2$ is approximated by 
 the variance $\tilde{\beta}_t$.

In conclusion, the reverse trajectory denoising process can be summarized as learning the Gaussian noise $\epsilon_\theta\left(\boldsymbol{x}_t, t\right)$ through $\boldsymbol{x}_t$ and $t$, and then solving $\mu_\theta\left(x_t, t\right)$ according to \cref{eq:mutheta}.
The stepwise denoising process is expressed as following equation:
\begin{equation}\label{eq:ptheta}
p_\theta\left(\boldsymbol{x}_{t-1} \mid \boldsymbol{x}_t\right)=\mathcal{N}\left(\boldsymbol{x}_{t-1} ; \frac{1}{\sqrt{\alpha_t}}\left(\boldsymbol{x}_t-\frac{1-\alpha_t}{\sqrt{1-\bar{\alpha}_1}} \boldsymbol{\epsilon}_\theta\left(\boldsymbol{x}_t, t\right)\right), \tilde{\beta}_t\mathbf{I}\right).
\end{equation}
Therefore, we can finally forge real-world-like trajectory data from random Gaussian with trained forward and backward processes.
% we can generate new trajectories from a random Gaussian by stepwise denoising with following equation:\notemar[02-02]{这一个section说的是reconstructing the trajectory。如果没有context，读者容易误以为你就是希望minimize reconstruction loss，与数据生成的目标不符。得在某个比较显眼的位置说明，reconstruction是手段，目标依旧是生成新数据，为什么这个手段可以生成新的、而不是重构原来的数据。}



% \begin{equation}\label{eq:invcond}
% \begin{aligned}
% q&\left(\boldsymbol{x}_t \mid \boldsymbol{x}_{t-1}, \boldsymbol{x}_0\right)=\frac{q\left(\boldsymbol{x}_{t-1} \mid \boldsymbol{x}_t, \boldsymbol{x}_0\right) q\left(\boldsymbol{x}_t \mid \boldsymbol{x}_0\right)}{q\left(\boldsymbol{x}_{t-1} \mid \boldsymbol{x}_0\right)}  \\
% &=\frac{\mathcal{N}\left(\boldsymbol{x}_t ; \sqrt{\alpha_t} \boldsymbol{x}_{t-1},\left(1-\alpha_t\right) \mathbf{I}\right) \mathcal{N}\left(\boldsymbol{x}_{t-1} ; \sqrt{\bar{\alpha}_{t-1}} \boldsymbol{x}_0,\left(1-\bar{\alpha}_{t-1}\right) \mathbf{I}\right)}{\mathcal{N}\left(\boldsymbol{x}_t ; \sqrt{\bar{\alpha}_t} \boldsymbol{x}_0,\left(1-\bar{\alpha}_t\right) \mathbf{I}\right)}
% \end{aligned}
% \end{equation}


\subsubsection{Objective Optimization Function}\label{sec:optim}
Recall that we need to approximate the conditional probability distribution $p_\theta\left(\boldsymbol{x}_{t-1} \mid \boldsymbol{x}_t\right)$ in the reverse trajectory denoising process. 
A typical method is to design a parameterized neural network model to predict the $\epsilon_\theta\left(\boldsymbol{x}_t, t\right)$ and implement this process by \cref{eq:ptheta}.
% \note[02-02]{need to design}{已经设计了还是还没有设计？这个和下一句的Therefore冲突。你如果要说会设计的，那就说这个地方我们先讲一下如果有了模型它应该怎么opt} a neural network to
% approximate the conditional probability distribution $p_\theta\left(\boldsymbol{x}_{t-1} \mid \boldsymbol{x}_t\right)$ in the reverse trajectory denoising process.
% We can optimize the denoising model by maximizing the log-likelihood between the predicted and original distributions as follows:
Since Diff-Traj contains two multi-step iteration processes, the design of the objective optimization function should guarantee desired results and is computationally efficient.
Thus, the objective optimization function can be derived by maximizing the log-likelihood between the predicted and original distributions, as follows.
\begin{align}
    \mathcal{L} = \mathbb{E}_{q(\boldsymbol{x}_0)}\left[-\log p_\theta\left(\boldsymbol{x}_0 \right) \right].
\end{align}
% \notemar[02-02]{一个一般性的建议，LaTeX中不要用equation和带eqn字样的环境。尽量全部只用align/aligned。比如下面这些公式，数字标号位置看上去有些奇怪，即使只有一个总的数字也应该是在最后一行末尾处。}
Similarly, the above formula can be optimized for negative log-likelihood by obtaining the variational lower bound based on variational inference \cite{ddpm}:
% We can optimize the negative log likelihood by obtaining the Variantional Lower Bound based on the variational inference \cite{ddpm}:
\begin{equation}\label{eq:lobjective}
\begin{aligned}
\mathcal{L} &\leq \mathbb{E}_q\left[-\log \frac{p_\theta\left(x_{0: T}\right)}{q\left(x_{1: T} \mid x_0\right)}\right] \\
% \mathcal{L} &= \mathbb{E}_{q(\boldsymbol{x}_0)}\left[-\log p_\theta\left(\boldsymbol{x}_0 \right) \right]\\
% &\leq \mathbb{E}_q\left[-\log \frac{p_\theta\left(x_{0: T}\right)}{q\left(x_{1: T} \mid x_0\right)}\right] \\
% &=\mathbb{E}_q\left[-\log p_\theta\left(x_T\right)-\sum_{t=1}^T \log \frac{p_\theta\left(x_{t-1} \mid x_t\right)}{q\left(x_t \mid x_{t-1}\right)}\right] \\
% &=\mathbb{E}_q\left[\log \frac{q\left(x_T \mid x_0\right)}{p_\theta\left(x_T\right)}+\sum_{t=2}^T \log \frac{q\left(x_{t-1} \mid x_t, x_0\right)}{p_\theta\left(x_{t-1} \mid x_t\right)}-\log p_\theta\left(x_0 \mid x_1\right)\right]\\
&\propto \mathbb{E}_q\left[\sum^T_{t=2} D_{K L}\left(q\left(x_{t-1} \mid x_t, x_0\right) \| p_\theta\left(x_{t-1} \mid x_t\right)\right)\right].
% &=\mathbb{E}_q\left[D_{K L}\left(q\left(x_T \mid x_0\right) \| p\left(x_T\right)\right)\right]-\log p_\theta\left(x_0 \mid x_1\right)\\
% & \quad \quad +\mathbb{E}_q\left[\sum^T_{t=2} D_{K L}\left(q\left(x_{t-1} \mid x_t, x_0\right) \| p_\theta\left(x_{t-1} \mid x_t\right)\right)\right].
\end{aligned}
\end{equation}
% where $\mathbb{E}_q\left[\log \frac{q\left(x_T \mid x_0\right)}{p_\theta\left(x_T\right)}\right]$ is a constant since $\boldsymbol{x}_T$ is Gaussian and $q(\cdot)$ has no learnable parameters.
% \begin{equation}
% L_{\text {simple }}(\theta)=\mathbb{E}_{t, x_0, \epsilon}\left[\left\|\epsilon-\epsilon_\theta\left(\sqrt{\bar{\alpha}_t} x_0+\sqrt{1-\bar{\alpha}_t} \epsilon, t\right)\right\|^2\right]
% \end{equation}
Therefore, the objective optimization function simplifies to:
\begin{equation}\label{eq:objf}
\begin{aligned}
\mathcal{L}& =\mathbb{E}_{\boldsymbol{x}_0, \boldsymbol{\epsilon}}\left[\frac{1}{2\left\|\boldsymbol{\Sigma}_\theta(\boldsymbol{x}_t,t)\right\|^2}\left\|\tilde{\boldsymbol{\mu}}_t\left(\boldsymbol{x}_t, \boldsymbol{x}_0\right)-\boldsymbol{\mu}_\theta\left(\boldsymbol{x}_t, t\right)\right\|^2\right] \\
& =\mathbb{E}_{x_0, \epsilon}\left[\frac{\beta_t^2}{2 \sigma_t^2 \alpha_t\left(1-\bar{\alpha}_t)\right)}\left\|\epsilon-\epsilon_\theta\left(\sqrt{\bar{\alpha}_t} x_0+\sqrt{1-\bar{\alpha}_t \epsilon}, t\right)\right\|^2\right]\\
&\propto \mathbb{E}_{t, x_0, \epsilon}\left[\left\|\epsilon-\epsilon_\theta\left(\sqrt{\bar{\alpha}_t} x_0+\sqrt{1-\bar{\alpha}_t} \epsilon, t\right)\right\|^2\right].
\end{aligned}
\end{equation}
The above equations show that the core of optimizing the diffusion model is to minimize the mean squared error between the Gaussian noise $\epsilon$ and predicted $\epsilon_\theta$.
% Details of the optimizing algorithm is summarized in \cref{alg:opt}. 


We give a detailed description of the optimization for Diff-Traj in \cref{alg:opt}.
We start by sampling a mini-batch real-world trajectories (line 2); next, we sample $t$ and $\epsilon$ from a uniform distribution and the standard Gaussian distribution, respectively (line 3); subsequently, we calculate the objective function $\mathcal{L}$ in \cref{eq:objf} (line 4); and finally, $\boldsymbol{\theta}$ is updated via descending 
 $\nabla_{\theta}\mathcal{L}$ (line 5). 
 The above steps are iterated until the objective function converges.
% and prediction model will introduce in \cref{sec:trajUNet}.


\begin{algorithm}[!t]
\caption{The Optimization for Diff-Traj.}\label{alg:opt}
\raggedright
{\bf Input}: Trajectories dataset $\boldsymbol{x} \in \mathcal{D}$ \\
{\bf Output}: Well-learned parameters of $\boldsymbol{\theta}^{*}$\\
\begin{algorithmic}[1]
% \textbf{Require}: Trajectory data $\mathcal{D}$, Denoising Model #o (), Timesteps I Noise schedule at\\
\WHILE{not converged} 
\STATE Sample a mini-batch of trajectories $\boldsymbol{x}_0 \sim q(\boldsymbol{x})$
\STATE $t \sim \operatorname{Uniform}\left\{1, \ldots, T \right\}$ and $\epsilon \sim \mathcal{N}(0, \mathbf{I})$
\STATE Calculate the objective via \cref{eq:objf}
\STATE  Update $\boldsymbol{\theta}$ by descending $\nabla_{\theta}\mathcal{L}$
\ENDWHILE
\end{algorithmic}
\end{algorithm}


% \note[02-02]{which is learned by a designed neural network}{读着就懵了。这个应该和3.1.4开头你说的那个是一个东西，但是没能呼应上。最好在前面就说明白我们需要个什么东西，干什么用的，后文会设计。} \cite{weng2021diffusion}.

\subsubsection{Speed up Diffusion Model Sampling}\label{sec:ddim}
As described in \cref{sec:noising} and \cref{sec:denoising}, Diff-Traj relies on a large Markov process to generate high-quality trajectories, rendering a slow reverse diffusion process.
To address this issue,  literature \cite{ddim} proposed a non-Markov diffusion process method with the same optimization objective, thus allowing a computationally efficient reverse process.
Specifically, following the reparameterization approach in \cref{eq:trick} and \cref{eq:forward}, we have
\begin{equation}\label{eq:ddimprocess}
\begin{aligned}
\boldsymbol{x}_{t-1} & =\sqrt{\bar{\alpha}_{t-1}} \boldsymbol{x}_0+\sqrt{1-\bar{\alpha}_{t-1}} \boldsymbol{\epsilon}_{t-1} \\
& =\sqrt{\bar{\alpha}_{t-1}} \boldsymbol{x}_0+\sqrt{1-\bar{\alpha}_{t-1}-\sigma_t^2} \boldsymbol{\epsilon}_t+\sigma_t \boldsymbol{\epsilon} \\
& =\sqrt{\bar{\alpha}_{t-1}} \boldsymbol{x}_0+\sqrt{1-\bar{\alpha}_{t-1}-\sigma_t^2} \frac{\boldsymbol{x}_t-\sqrt{\bar{\alpha}_t} \boldsymbol{x}_0}{\sqrt{1-\bar{\alpha}_t}}+\sigma_t \boldsymbol{\epsilon}.
\end{aligned}
\end{equation}
Then, we can sample every $\left \lceil T/S \right \rceil $ steps with the skip-step method presented in \cite{nichol2021improved}.
The corresponding set of noise trajectories changes to $\left\{\tau_1, \ldots, \tau_S\right\}, \tau_i \in \left[1, T\right]$.
Through this approach, the sampling steps during trajectory generation can be significantly reduced from $T$ steps to $S$ steps.
Therefore, the reverse denoising process of \cref{eq:cond} is rewritten as:
% \note[02-02]{it}{who?} follows the skip-step sampling schedule in \fix{literature}{} \cite{nichol2021improved}\fix{, sampling}{ and samples} every $\left \lceil T/S \right \rceil $ steps, thus reducing the number of steps in the entire process from $T$ steps to $S$ steps.\notemar[02-02]{左边这句没头没尾，文法读起来也很乱。重写}
% So, the new \note[02-02]{generation schedule}{这是啥？看上去是Markov的东西，但是不一定读者对这方面很熟悉。得考虑换一种方式表达} is $\left\{\tau_1, \ldots, \tau_S\right\}, \tau_i \in \left[1, T\right]$.
% The reverse denoising is expressed as:
\begin{equation}\label{eq:ddim}
   q_{\sigma,\tau}\left(\boldsymbol{x}_{\tau_i-1} \mid \boldsymbol{x}_t, \boldsymbol{x}_0\right)=\mathcal{N}\left(\sqrt{\alpha_{t-1}} \boldsymbol{x}_0+\sqrt{1-\alpha_{t-1}-\sigma_t^2} \frac{\boldsymbol{x}_{\tau_i}-\sqrt{\alpha_t} \boldsymbol{x}_0}{\sqrt{1-\alpha_t}}, \sigma_t^2 \boldsymbol{I}\right). 
\end{equation}
Unlike \cref{eq:qxtx0} and \cref{eq:mutheta}, \cref{eq:ddim} introduces variance $\sigma_t^2$ into the mean of Gaussian.
Let $\sigma_t^2 =\eta \tilde{\beta}_t$, where $\eta \in \mathbb{R}$ is a hyperparameter that controls sampling randomness. 
% $\eta = 1$ means no changes added for diffusion model
% \fix{When $\eta=1$, i.e., $\sigma_t^2 = \tilde{\beta}_t =\frac{1-\bar{\alpha}_{t-1}}{1-\bar{\alpha}_t} \beta_t$}{
In such a case, \cref{eq:ddim} is equivalent to \cref{eq:qxtx0} when $\eta=1$, i.e., $\sigma_t^2 = \tilde{\beta}_t =\frac{1-\bar{\alpha}_{t-1}}{1-\bar{\alpha}_t} \beta_t$.
On the other hand, the sampling process of diffusion loses all randomness to obtain a deterministic result when $\eta=0$.
Compared to the typical diffusion model \cite{ddpm}, this method can generate higher quality samples in fewer steps \cite{ddim}.
% \zxy{add an optimization algorithm table, and line-wise description of it, refer to AutoLoss}



% and \cref{eq:ddim} is equivalent to \cref{eq:qxtx0} when $\sigma_t^2 = \tilde{\beta}_t & =\frac{1-\bar{\alpha}_{t-1}}{1-\bar{\alpha}_t} \beta_t$.
% Based on this formulation, the reverse denoising is written as:
% \begin{equation}
% \begin{aligned}
% \boldsymbol{x}_{t-1} & =\sqrt{\alpha_{t-1}}\left(\frac{\boldsymbol{x}_{t}-\sqrt{1-\alpha_{t}} \epsilon_\theta\left(\boldsymbol{x}_{t},t\right)}{\sqrt{\alpha_{t}}}\right) \\
% & +\sqrt{1-\alpha_{t-1}-\sigma_{t}} \cdot \epsilon_\theta\left(\boldsymbol{x}_{t},t\right) \\
% & +\sigma_{t} \epsilon.
% \end{aligned}
% \end{equation}

% \begin{equation}
% \begin{aligned}
%    \mathbf{x}_{t-1} &=\sqrt{\alpha_{t-1}}(\underbrace{\left.\frac{\mathbf{x}_t-\sqrt{1-\alpha_t} \epsilon_\theta\left(\mathbf{x}_t, t\right)}{\sqrt{\alpha_t}}\right)}_{\text {predicted } \mathbf{x}_0}+\underbrace{\sqrt{1-\alpha_{t-1}-\sigma_t^2} \cdot \epsilon_\theta\left(\mathbf{x}_t, t\right)}_{\text {direction pointing to } \mathbf{x}_t}\\
%    &+\underbrace{\sigma_t \epsilon_t}_{\text {random noise }} 
% \end{aligned}
% \end{equation}

% \begin{equation}
% \sigma_t= \eta \sqrt{\frac{1-\alpha_{t-1}}{1-\alpha_t}} \sqrt{\frac{1-\alpha_t}{\alpha_{t-1}}}.
% \end{equation}

% $\eta = 1$ means no changes added





\subsection{Coupled Traj-UNet for Denoising}\label{sec:trajUNet}




In \cref{sec:diffModel}, we have introduced the theoretical foundation of Diff-Traj framework, i.e., the forward trajectory noising and reverse trajectory denoising processes.
In this section, we present the proposed neural network model to learn the noise $\epsilon_{\theta}$, assisting the reverse trajectory denoising process.
Typically, the denoising network for the diffusion model follows the UNet structure \cite{unet,diffusionsuvery}, with the input being the time step $t$ and the corresponding noise sample, and outputting Gaussian noise corresponding to $\boldsymbol{x}_t$.
% In this paper, we proposed the trajectory UNet structure for denoising in trajectory generation.
Unlike the traditional structure presented in \cite{unet}, Traj-UNet incorporates time steps and traffic contextual information for each down/up-sampling blocks, as well as 1D convolutions to capture fine-grained spatio-temporal features.
As illustrated in \cref{fig:structure}, Traj-UNet is divided into two modules, i.e., down-sampling and up-sampling, each consisting of multiple stacked Resnet blocks.
Between the two modules, a transitional module based on the attention mechanism is integrated \cite{vaswani2017attention}.
To better learn the noise of each time step, Traj-UNet embeds the time step and external traffic information, later fed to each block.

\subsubsection{Component Blocks}
As previously stated, Traj-UNet consists of several blocks with different architectures and functionalities. 
We first detail the role and design of each block depicted in \cref{fig:blocks}.

\textbf{Sampling Block.} 
This is the most essential component of Traj-UNet.
As illustrated in \cref{fig:structure}, the sampling blocks (both down- and up-sampling) consists of multiple Resnet blocks, each containing a series of group normalization, nonlinear activation, and 1D convolutional layers.
% As is illustrated in  each sampling consists of multiple resnet blocks, each comprising a series of group normalization, nonlinear activation and 1D convolutional layers (see \cref{fig:blocks} for details).
For a given input $\mathbf{X} \in \mathbb{R}^{ c \times n}$
($c$ and $n$ represent the dimensions and length of the acquired trajectory features, respectively), the Resnet block can be formulated as:
% ($c$ represents the \note[02-02]{dimensions and $n$ represents the length}{对于轨迹来说是什么？}), the \note[02-02]{resnet}{} block can be formulated as:
\begin{equation}\label{eq:sampling}
\begin{aligned}
    \mathbf{X}^{l} &= \operatorname{Conv}(\sigma(\operatorname{GN}(\mathbf{X}^{l-1}))),\\
    \mathbf{X}^{l} &= \mathbf{X}^{l} + \operatorname{Concat}(\operatorname{Embed}(t) , \operatorname{Embed}(Attr)),\\
    \mathbf{X}^{l} &= \operatorname{Conv}(\sigma(\operatorname{GN}(\mathbf{X}^{l}))),\\
    \mathbf{X}^{l} &= \mathbf{X}^{l} + \mathbf{X}^{l-1},
\end{aligned}
\end{equation}
where $\sigma(\cdot)$ is the nonlinear activation function.
For each Resnet block, we use a skip connection to join the output of the convolutional layer with the input features from the same level.
This design permits the model to capture spatial-temporal features at different resolutions and skip connections to facilitate the addition of trajectory details.
After this, Traj-UNet applies up-sampling or down-sampling to the output, where down-sampling uses maximum-pooling and up-sampling uses interpolation.

\begin{figure}[!t]
    \includegraphics[width=0.9\linewidth]{Figures/Blocks.pdf}
    \caption{The main components of Traj-UNet including Resnet block, embed block, attention layer, and middle attention block.}
    \label{fig:blocks}
    % \vspace{-6mm}
\end{figure}
% In addition, 
% After each connection, we apply an attention layer to enable the model to learn more accurate output features.

% \begin{table*}[t]
%     \caption{Performance Comparison of Different Approaches.   }
%     % \small
%     \centering
%     \begin{tabular}{llcccccccccc} 
%     \toprule
%     \multirow{2}{*}[\multirowoffset]{Types} & \multirow{2}{*}[\multirowoffset]{Methods} & \multicolumn{5}{c}{Chengdu} & \multicolumn{5}{c}{Xi'an}  \\
%     \cmidrule(lr){3-7}\cmidrule(lr){8-12}
%     &  & MMR & JS-Traj & JS-O & JS-D & JS-Dis & MMR & JS-Traj & JS-O & JS-D & JS-Dis \\ 
%     \cmidrule(lr){1-12}
%    \multirow{2}{*}{Non-generative} & RP  & 85.82\% & 0.0358 & 0.0245 & 0.0263 & 0.1933 & 51.54\%  & 0.0157 & 0.0174& 0.0166 & 0.2157 \\
%     & GP  & 81.76\% & 0.0203 & 0.0237 & 0.0265 & 0.1918 & 47.35\% & 0.0216  &0.0234 & 0.0213 &0.1937\\
%     % & DP  &  &  &  &  &  &  &  &\\
%     \cmidrule(lr){1-12}
%     \multirow{5}{*}{Generative} & VAE  & 88.33\% & 0.0079 & 0.0070 & 0.0085 & 0.0255&67.11\%  & 0.0131 & 0.0136 & 0.0209  & 0.0491\\
%     & TrajGAN  & 89.92\% & 0.0074 & 0.0072 & 0.0079 & 0.0285 & 56.64\% &0.0181  & 0.0160 &0.0198 &0.0638\\
%     % & SeqGAN  &  &  &  &  &  &  &  &\\
%     & Diff-scatter  & --  & 0.0170 & 0.0157 & 0.0122 &--  &  --  &0.0267 &0.0286 & 0.0329 &-- \\
%     & Diff-wo/Traj-UNet  &  90.72\% & 0.0046 & 0.0134 & 0.0161 &  0.0245 & 75.83\%  & 0.0109  &  0.0219 & 0.0158 &0.0084\\
%     & Diff-Traj  &  \textbf{95.39\%} & \textbf{0.0027} & \textbf{0.0053} & \textbf{0.0035} &  \textbf{0.0071} & \textbf{82.15\%}  & \textbf{0.0065} &  \textbf{0.0079} & \textbf{0.0076} & \textbf{0.0042} \\
   
%     \bottomrule
%     \end{tabular}
%     \label{tab:comp}
% \\ 
% Bold indicates the statistically best performance (i.e., two-sided t-test with $p$ < 0.05) over the best baseline.
% % \zxy{significance test against the best baseline, refer to AutoLoss}
% \end{table*}



\textbf{Middle Attention Block.} 
After the capture spatial-temporal features capturing by down- and up-sampling modules, 
Traj-UNet needs to determine the importance of its high-dimensional features to improve the accuracy and efficiency of the generation process.
To address this issue, Traj-UNet integrates a middle attention block. 
As shown in \cref{fig:blocks}, it consists of two Resnet blocks and an attention layer.
Note that there are no additional down-/up-sampling operations in the Resnet block.
In Traj-UNet, the attention layer can be formulated as follows:
\begin{equation}
\begin{aligned}
    \operatorname{Attention}(\mathbf{Q}, \mathbf{K}, \mathbf{V})&=\operatorname{softmax}\left(\frac{\mathbf{Q} \mathbf{K}^{\top}}{\sqrt{d}}\right) \cdot \mathbf{V}, \\
    \mathbf{X}^{l+1} &=\mathbf{X}^{l} + \operatorname{Attention}(\mathbf{Q}, \mathbf{K}, \mathbf{V}),
\end{aligned}
\end{equation}
 where $\mathbf{Q}=\mathbf{W}_Q^{l} \cdot \mathbf{X}^{l},~ \mathbf{K}=\mathbf{W}_K^{l} \cdot \mathbf{X}^{l},~ \mathbf{V}=\mathbf{W}_V^{l} \cdot \mathbf{X}^{l}$ ($\mathbf{W}_Q, \mathbf{W}_K$, and $\mathbf{W}_V$ are learnable parameter matrices).

The motivation of this design is to first use the Resnet block to learn the high-dimensional spatio-temporal features after down-sampling.
The subsequent calculation of the feature importance through attention ensures that data are propagated with efficacy.
Finally, Traj-UNet integrates this information with a Resnet block to facilitate the subsequent up-sampling module.

% \textbf{Attention Layer.}
% Attention is a common technique that allows models to focus on and learn important information sufficiently, which can be integrated into any neural network models \cite{vaswani2017attention}.
% In the diffusion model, attention determines the important fine-grained features to be shared and transmitted, which helps ensure that information is propagated in an efficient and effective manner \cite{diffusionsuvery}.
% \zxy{challenges}
% For trajectory generation tasks, attention can help to identify the most important component of a trajectory sequence, leading to better capture of spatio-temporal features.
% In Traj-UNet, the attention layer can be formulated as:
% \begin{equation}
% \begin{aligned}
%     \operatorname{Attention}(\mathbf{Q}, \mathbf{K}, \mathbf{V})&=\operatorname{softmax}\left(\frac{\mathbf{Q} \mathbf{K}^{\top}}{\sqrt{d}}\right) \cdot \mathbf{V}, \\
%     \mathbf{X}^{l+1} &=\mathbf{X}^{l} + \operatorname{Attention}(\mathbf{Q}, \mathbf{K}, \mathbf{V}),
% \end{aligned}
% \end{equation}
%  where $\mathbf{Q}=\mathbf{W}_Q^{l} \cdot \mathbf{X}^{l},~ \mathbf{K}=\mathbf{W}_K^{l} \cdot \mathbf{X}^{l},~ \mathbf{V}=\mathbf{W}_V^{l} \cdot \mathbf{X}^{l}$ ($\mathbf{W}_Q, \mathbf{W}_K$, and $\mathbf{W}_V$ are learnable parameter matrices).
% % 可以看到不同分辨率的特征，并且跳过连接有利于添加图像的细节
% % 为了获得更精确的位置，在解码器的每一步，我们都使用跳过连接，将转置卷积层的输出与来自同一级别的编码器的特征映射连接起来：
% % 在每次连接之后，我们再次应用两个连续的常规卷积，以便模型可以学习组装更精确的输出
% After calculating the attention of the high-dimensional trajectory features, Traj-UNet applies up-sampling or down-sampling to the output, where down-sampling uses maximum-pooling and up-sampling uses interpolation.


\subsubsection{Time Step and External Attribute Embedding} 
Encoding time step $t$ in Diff-Traj is necessary, which is because the diffusion model generates trajectories using a probabilistic approach, requiring it to consider the current state of the trajectory at each time step.
% Since the denoising model needs to output $\epsilon_\theta\left(\boldsymbol{x}_t, t\right)$ for different $t$, we 
% incorporate the diffusion step index $t$ as part of the input. 
In this work, we encode each $t$ using a $128$-dimensional vector according to the method in literature \cite{vaswani2017attention}.
We then apply two fully connected layers on the encoding and superimpose the result to the input of each Resnet block:
\begin{equation}
    t_{\text{emb}} = \operatorname{FC}(\sigma( \operatorname{FC}(\operatorname{SinTimeEmb}(t)))),
\end{equation}
where $\operatorname{FC}$ denotes fully connected layer and $\operatorname{SinTimeEmb}$ is the step index encoding following \cite{vaswani2017attention}.


In addition, external attributes have a non-negligible impact on the dynamics of the GPS trajectory \cite{WDR, DeepTTE}.
We consider the effects of travel distance, average move distance, and the departure time of the trajectory.
Specifically, we adopt linear transformations with biases to embed categorical features $x$ (i.e., departure time) into low-dimensional vectors of $\mathbb{R}^{128}$. 
Here, we divide the departure time during the day into $288$ slices (\SI{5}{\minute} for each time window).
For the travel distance and average move distance, we apply the z-score for normalization.
After obtaining all external attribute embedding, a fully connected layer is adopted to map them to the same dimensions of the time step embedding for data aggregation. 
% \fix{With the above neural network components, we can build deep learning models (Traj-UNet) to capture potential features and combine time steps to predict the noise of each step.}{}




% \begin{algorithm}[!t]
% 	\caption{cross-area travel time uncertainty estimation algorithm}\label{alg:catte}
	
% 	\textbf{Input:}  \\~~~~{Order ID $\mathcal{O}$, travel trajectory $\mathcal{P}$.}\\
%         	~~~~{Center server $\mathcal{S}_c$, Area server set $\left\{ \mathcal{S}_{1}, \ldots, \mathcal{S}_{m}\right\}$.}\\
% 	\textbf{Output:}  \\~~~~{Estimated travel time distribution $\mathcal{T}$.}\\
% 	\textbf{User}:  
% 	\begin{algorithmic}[1]
% 	\STATE {Split the trajectory $\mathcal{P}$ into $n$ ($n < m$) segments $\left\{P_1, \ldots, P_n\right\}$ based on the local map}
% 	\STATE {Encrypt the order ID \\$\left\{O_1, \ldots, O_n\right\}$ $\leftarrow$ \textbf{Encrypt}($\mathcal{O}$).}\\
% 	\STATE {Send trajectory segments and encrypted order pairs $\left\{(P_1,O_1),\ldots,(P_i,O_i) \right\}$ to the central server.}
%     \end{algorithmic}	
%     \textbf{Center Server:}\\
% 	\begin{algorithmic}[1]
% 	\STATE {Receives the segment and order pairs.}
% 	\STATE {Send pairs to the corresponding area server $\left\{ \mathcal{S}_{1}, \ldots, \mathcal{S}_{n}\right\}$.}
% 	\end{algorithmic}
% 	\textbf{Area Server:}\\
% 	\begin{algorithmic}[1]
% 	\FOR{area server $\mathcal{S}_a \in \left\{ \mathcal{S}_{1}, \ldots, \mathcal{S}_{n}\right\}$, \textbf{in parallel}} 
% 	\FOR{Monte-Carlo sample $i=1, \ldots, M$}
% 		\STATE $t_i$ $\leftarrow$ \textbf{AreaModel}($P_i$, w)
% 		\STATE add $t_i$ to the set of estimated values $\mathcal{T}_a$.
% 	\ENDFOR
% 	\STATE {send $\mathcal{T}_a=\left\{t_1, \ldots, t_M \right\}$ and encrypted \\order ID $O_i$ to the center server.}
%     \ENDFOR
% 	\end{algorithmic}
% 	\textbf{Center Server:}\\
% 	\begin{algorithmic}[1]
% 	\STATE {Receives all estimated $\left\{\mathcal{T}_1,\ldots,\mathcal{T}_n \right\}$ of areas and encrypted order ID.}
% 	\STATE {Cross-merge and sum the estimates from different segment\\ $\mathcal{T}$ $\leftarrow$ \textbf{sum}($\left\{\mathcal{T}_1,\ldots,\mathcal{T}_n \right\}$)}
% % 	\STATE {$T$ $\leftarrow$ \textbf{mean}($\mathcal{T}$),~~$\sigma$ $\leftarrow$ \textbf{var}($\mathcal{T}$).}
% 	\STATE {Reconstruct the order ID \\$\mathcal{O}$ $\leftarrow$  \textbf{Decrypt}($\left\{O_1, \ldots, O_n\right\}$)}
% 	\STATE Send estimated travel time distribution $\mathcal{T}$ back to \\the user according to the order ID $\mathcal{O}$
% 	\end{algorithmic}
% \end{algorithm}

==> 05-Experimentsback.tex <==

% \begin{table*}[t]
%     \caption{Performance Comparison of Different Approaches.   }
%     \footnotesize
%     \centering
%     \begin{tabular}{llcccccccc} 
%     \toprule
%     \multirow{2}{*}[\multirowoffset]{Types} & \multirow{2}{*}[\multirowoffset]{Methods} & \multicolumn{4}{c}{Chengdu} & \multicolumn{4}{c}{Xi'an}  \\
%     \cmidrule(lr){3-6}\cmidrule(lr){7-10}
%     &  & MMR & JS-Traj & JS-OD  & JS-Dis & MMR & JS-Traj & JS-OD & JS-Dis \\ 
%     \cmidrule(lr){1-10}
%    \multirow{2}{*}{Non-generative} & RP  & 85.82\% & 0.0358 & 0.0245 & 0.1933 & 51.54\%  & 0.0157 & 0.0174 & 0.2157 \\
%     & GP  & 81.76\% & 0.0203 & 0.0237  & 0.1918 & 47.35\% & 0.0216  &0.0234  &0.1937\\
%     % & DP  &  &  &  &  &  &  &  &\\
%     \cmidrule(lr){1-10}
%     \multirow{5}{*}{Generative} & VAE  & 88.33\% & 0.0079  & 0.0085 & 0.0255&67.11\%  & 0.0131 & 0.0136  & 0.0491\\
%     & TrajGAN  & 89.92\% & 0.0074 & 0.0072 & 0.0079  & 56.64\% &0.0181  & 0.0160 &0.0638\\
%     % & SeqGAN  &  &  &  &  &  &  &  &\\
%     & Diff-scatter  & --  & 0.0170 & 0.0157  &--  &  --  &0.0267 &0.0286  &-- \\
%     & Diff-wo/Traj-UNet  &  90.72\% & 0.0046 & 0.0134  &  0.0245 & 75.83\%  & 0.0109  &  0.0219 &0.0084\\
%     & Diff-Traj  &  \textbf{95.39\%} & \textbf{0.0030} & \textbf{0.0052}  &  \textbf{0.0071} & \textbf{82.15\%}  & \textbf{0.0065} &  \textbf{0.0079} & \textbf{0.0042} \\
   
%     \bottomrule
%     \end{tabular}
%     \label{tab:comp}
% \\ 
% Bold indicates the statistically best performance (i.e., two-sided t-test with $p$ < 0.05) over the best baseline.
% % \zxy{significance test against the best baseline, refer to AutoLoss}
% \end{table*}


\begin{table*}[t]
    \caption{Performance Comparison of Different Approaches.   }
    \footnotesize
    \centering
    \begin{tabular}{lcccccccc} 
    \toprule
      \multirow{2}{*}[\multirowoffset]{Methods} & \multicolumn{4}{c}{Chengdu} & \multicolumn{4}{c}{Xi'an}  \\
    \cmidrule(lr){2-5}\cmidrule(lr){6-9}
     & MMR & JS-Traj & JS-OD  & JS-Dis & MMR & JS-Traj & JS-OD & JS-Dis \\ 
    \cmidrule(lr){1-9}
   RP  & 85.82\% & 0.0358 & 0.0245 & 0.1933 & 51.54\%  & 0.0157 & 0.0174 & 0.2157 \\
    GP  & 81.76\% & 0.0203 & 0.0237  & 0.1918 & 47.35\% & 0.0216  &0.0234  &0.1937\\
    % & DP  &  &  &  &  &  &  &  &\\
    \cmidrule(lr){1-9}
      VAE  & 88.33\% & 0.0079  & 0.0085 & 0.0255&67.11\%  & 0.0131 & 0.0136  & 0.0491\\
     TrajGAN  & 89.92\% & 0.0074 & 0.0072 & 0.0079  & 56.64\% &0.0181  & 0.0160 &0.0638\\
    % & SeqGAN  &  &  &  &  &  &  &  &\\
     Diff-scatter  & --  & 0.0170 & 0.0157  &--  &  --  &0.0267 &0.0286  &-- \\
    Diff-wo/Traj-UNet  &  90.72\% & 0.0046 & 0.0134  &  0.0245 & 75.83\%  & 0.0109  &  0.0219 &0.0084\\
    Diffwave  &  &  &  &  &  &  &  & \\
    DiffTraj-LSTM  &  &  &  &  &  &  &  & \\
    Diff-wo/Traj-UNet  &  90.72\% & 0.0046 & 0.0134  &  0.0245 & 75.83\%  & 0.0109  &  0.0219 &0.0084\\
 Diff-Traj  &  \textbf{95.39\%} & \textbf{0.0030} & \textbf{0.0052}  &  \textbf{0.0071} & \textbf{82.15\%}  & \textbf{0.0065} &  \textbf{0.0079} & \textbf{0.0042} \\
   
    \bottomrule
    \end{tabular}
    \label{tab:comp}
\\ 
Bold indicates the statistically best performance (i.e., two-sided t-test with $p$ < 0.05) over the best baseline.
% \zxy{significance test against the best baseline, refer to AutoLoss}
\end{table*}



\section{Experiments}\label{sec:exper}
In this section, a series of comprehensive experiments on two real-world trajectory datasets are conducted to show the superiority of the proposed Diff-Traj.
% we conduct extensive experiments on two real-world trajectory datasets to investigate the performance of the proposed Diff-Traj.
We first introduce the public datasets and evaluation metrics used in this paper.
Subsequently, we briefly review selected baselines and experimental details.
Finally, we analyze and discuss the result of Diff-Traj by extensive experiments.

% chengdu 99.41  xian 9307



\begin{figure*}[!t]
    \centering
    \subfigure[VAE]{
        \includegraphics[width=0.14\linewidth]{Figures/traj_chengdu_vae.pdf}
        % \label{fig:noising}
    }
    \subfigure[Traj-GAN]{
        \includegraphics[width=0.14\linewidth]{Figures/traj_chengdu_gan.pdf}
        % \label{fig:noising}
    }
    \subfigure[Diff-scatter]{
        \includegraphics[width=0.14\linewidth]{Figures/traj_chengdu_scatter.pdf}
        \label{fig:diffscatter}
    }
    \subfigure[Diff-wo/Traj-UNet]{
        \includegraphics[width=0.14\linewidth]{Figures/traj_chengdu_mlp.pdf}
        \label{fig:diffunet}
    }
    % \quad 
    \subfigure[Diff-Traj]{
        \includegraphics[width=0.14\linewidth]{Figures/traj_chengdu_ddpm.pdf}
        \label{fig:difftraj}
    }
      \subfigure[Real]{
        \includegraphics[width=0.14\linewidth]{Figures/traj_chengdu_ori.pdf}
        \label{fig:gen-original}
    }
    \caption{Comparison of forged trajectory in Chengdu.}
    \label{fig:resultcompchengdu}
    % \vspace{-3mm}
\end{figure*}


\subsection{Experimental Settings}\label{sec:expsetting}



\subsubsection{Data and Configuration}\label{sec:config}
We evaluate the generative performance of Diff-Traj and baselines on two real-world trajectory datasets of Chinese cities, namely, Chengdu and Xi'an.
Both datasets are collected from cab trajectory data starting from November 1, 2016 to November 30, 2016.
A detailed description of the dataset and statistics is available in \cref{app:dataset}.



\subsubsection{Evaluation Metrics}
As trajectory generation aims to generate trajectories that can replace real-world activities and further benefit downstream tasks, we need to evaluate the ``similarity'' between the forged trajectories and real ones.
In this work, we follow the common practice in previous studies \cite{feng2020learning,luca2021survey} and measure the quality of the forged ones by JSD. 
JSD compares the distribution of the real and forged trajectories, and a lower JSD indicates a better match with the original statistical features (see \cref{sec:pre} for details).
We adopt the following metrics to evaluate the quality of the forged trajectories from four perspectives:
\begin{itemize}[leftmargin=*]
    \item \textbf{Trajectory Distribution (JS-Traj):} This metric is used to evaluate the geo-distribution between the entire forged trajectory and the real trajectory.

    \item \textbf{Origin Distribution (JS-O):} In addition to evaluating the trajectory distribution, this metric is adopted to assess the geo-distribution of trajectory origins.

    \item \textbf{Destination Distribution (JS-D):} This metric is used to evaluate the geo-distribution of trajectory destinations.
    
    \item \textbf{Travel Distance Distribution (JS-Dis):}  This metric evaluates the distribution of travel distances.
    
\end{itemize}   
% In addition, it is also essential to identify whether the forged trajectories match the road network, as it indicates the consistency of the forged trajectories and the real-world patterns.
In addition, since map matching is a common pre-processing step in various applications, it is essential to identify whether forged trajectories match well with the road network.
Thus, the following metric is used to evaluate the quality and utility of forged trajectories:
\begin{itemize}[leftmargin=*]
    \item \textbf{Map Matching Rate (MMR):} This work adopts the fast map matching approach for map matching \cite{fmm}, where a higher MMR indicates that the forged trajectories are more consistent with the real-world spatial distribution of the road network and in turn human activities.
\end{itemize}


\subsubsection{Implementation Details}
The Diff-Traj implementation is based on PyTorch $3.7$ \cite{pytorch}, which involves various general neural network components. The implementation is available at \url{https://anonymous.4open.science/r/Diff-Traj-875A/}. See \cref{app:imple} for detailed hyperparameter settings and implementation details. 




\subsubsection{Baseline Methods}
We compare Diff-Traj with two categories of baselines: non-generative and generative methods.
The details of the implementation are presented in \cref{app:baseline}.

\noindent\textbf{Non-generative:} 
\begin{itemize}[leftmargin=*]
    \item \textbf{Random Perturbation (RP): }
    Random perturbation is a method to preserve the privacy of trajectories, where each location moves in planar space at a randomly determined distance and direction. 

    \item \textbf{Gaussian Perturbation (GP): }
    Gaussian perturbation is a geo-masked privacy-preserving method, where it replaces the real location with noise sampled from the Gaussian.
    % \notemar[02-02]{为什么没有DP？很可能被问到}

    % \item \textbf{Differential Privacy (DP): }
    % Differential privacy is a cryptography method, which adds multiple alternative locations  within a range to protect the individual privacy.
\end{itemize}
\textbf{Generative:} Please note that Diff-scatter and Diff-wo/UNet can be considered as \textbf{ablation studies} of the proposed method to evaluate the functions of the diffusion model and Traj-UNet, respectively.
\begin{itemize}[leftmargin=*]
    \item \textbf{Variational AutoEncoder (VAE): }  VAE is a common data generation method, which learns data representations through an encoder and then reconstructs it by a decoder \cite{liou2014autoencoder}. 

    \item \textbf{TrajGAN: } TrajGAN is a GAN-based framework for trajectory generation. By alternately training the generator and discriminator, it eventually enables its generated data to be consistent with the distribution of the real data \cite{Gan}.
    
    \item \textbf{Diff-scatter: } This method uses a diffusion model to directly generate scatter points of trajectories, which can be used to evaluate the ability of a typical diffusion model on learning citywide trajectory distribution.

    \item \textbf{Diff-wo/Traj-UNet: } This method is a variant of Diff-Traj without Traj-UNet, which can be used to evaluate the effectiveness of the proposed Traj-UNet spatial-temporal extraction capability.
    
\end{itemize}

\subsection{Overall Performance}

% 画出生成的地图结果图，最好情况，别的只能生成一部分，而我们的能生成所有地区。
\cref{tab:comp} presents the performance comparison of
Diff-Traj and the selected baseline methods on two real-world datasets.
Specifically, we randomly generate $1000$ trajectories from each generative method and then compare their distribution with the real ones.
In addition,  we directly perturb the real trajectory and then calculate all metrics for each non-generative approach.
Note that Diff-scatter generates scattered points and therefore cannot be applied with MMR or JS-Dis.
The following conclusions can be derived from the performance comparison:
\begin{itemize}[leftmargin=*]
    
    \item The non-generative approaches protect privacy by perturbing the raw trajectory, but they inevitably impair the real trajectory properties.
    Compared to generative ones, they are inferior in all metrics. 
    In particular, the non-generative approach demonstrates a poor result in JS-Dis due to data perturbations corrupting the motion feature within the trajectory.
    
    % 非生成式方法
    \item Generative methods generate trajectories directly and maintain the statistical properties of the real data.
    Among them, Diff-Traj achieved the best performance in all metrics.
    Its remarkable superiority can be attributed to the unique forward and backward diffusion processes incorporated in the model, which help better learn the distribution of trajectories.
    Such results advocate the employment of diffusion models in future studies related to spatial-temporal data generation.
    In addition, Diff-Traj significantly outperforms other methods on the JS-Dis metric, which indicates its ability to generate more realistic human activities.
    
    \item VAE and GAN outperform Diff-scatter and Diff-wo/Traj-UNet in some metrics, but Diff-Traj achieves optimal results when Traj-UNet is integrated.
 It is also noteworthy that satisfactory results can still be accomplished when using only MLP to generate scattered locations or discarding Traj-UNet structure.
    % Thanks to the strong ability of the diffusion model, satisfactory results can still be accomplished when using only MLP to generate scattered locations or discarding Traj-UNet structure.
    % \note[02-02]{}{这里少了个转折。前面说diffusion自己就挺好的，后面一句就说VAE和GAN比单独diffusion好。这个很明显要说你加进去的东西是essential的}
    % Although VAE and GAN outperform Diff-scatter and Diff-wo/Traj-UNet in some metrics, Diff-Traj achieves optimal results when Traj-UNet is integrated.
    Such results may be attributed to two reasons:
    \begin{enumerate}
        \item Traj-UNet is equipped with outstanding generation capabilities, which is able to generate trajectories consistent with the original distribution even by the simplest models and data.      
        % Traj-UNet stacks multiple Resnet blocks to capture the spatial-temporal features of the trajectory, then it captures fine-grained information from different dimensions by down-sampling and up-sampling.
        % \note[02-02]{}{为什么用resent和上下采样就比VAE等更好？给个直观的原因。没有说服力}
        \item Diff-Traj equipped with Traj-UNet benefits from stacking multiple Resnet blocks and skip connections, enabling it to learn spatio-temporal features and capture trajectory details at different resolutions.
    % (ii) The diffusion model recovers the real data by step-wise denoising from Gaussian, whereas the \note[02-02]{powerful}{outstanding} spatial-temporal modeling capability of Traj-UNet can accurately predict the noise at each step.\note[02-02]{}{同上，没啥说服力。}
    \end{enumerate}
    % \note[02-02]{}{继续缩进，itemize或者enumerate哪个好看用哪个。}
    
\end{itemize}
% 图表解释 地图可视化  
% 首先介绍性能表现，表1，先介绍轨迹分布，JS-Traj 和JS-OD,然后介绍JS-Dis, 最后是MMR。 若有特殊实例，要解释
To summarize, Diff-Traj relies on diffusion models and Traj-UNet to forge trajectories where the former simulates the geo-distribution of trajectories and the latter significantly improves the quality of results over existing approaches.

\begin{figure}[!t]
% \vspace{-10mm}
    \includegraphics[width=\linewidth]{Figures/compare_dis_chengdu.pdf}
    % \vspace{-6mm}
    \caption{Comparison of the real and forged trajectory distributions.
    The city is divided into different size grids (from left to right, $32\times32$, $16\times16$, and $8\times8$ grids).}
    \label{fig:compchengdudis}
     \vspace{-6mm}
\end{figure}


\subsection{Geographic Visualization}
In this section, we visualized the forged results to better present the performance of different generative models.
% \note[02-02]{To better present the performance of different generative models, we visualized their generated results.}{写英文的时候要注意，这类的"为了XXX所以XXX"，一个自然的英文语序应该是"我们做了XXX用以XXX"。也就是说，这类倒装都应该反过去说，除非你的目的特别的与众不同想要格外强调。} 
\cref{fig:resultcompchengdu} shows the trajectory distributions generated by baseline methods for Chengdu (The results of Xi'an are available in \cref{fig:genxian} at \cref{app:visu}).
\cref{fig:compchengdudis} compares the heat map between real trajectories and forged ones.
According to the results shown
% \note[02-02]{results shown}{一个自然的问题：原始数据为什么不可视化？要有一个强的理由。} 
in \cref{fig:resultcompchengdu}, the trajectory data generated from VAE, Traj-GAN, and Diff-Traj are approximately identical to geo-distribution compared to original ones.
% \note[02-02]{urban trajectory geographical distribution conditions}{看不懂，google一下有没有专业词汇描述这个东西。}.
Notably, the trajectories generated by Diff-Traj best resemble the road network without obvious offsets.
The superior data generation capability of the diffusion model is further validated in \cref{fig:diffscatter}, where the diffusion model can yield a similar distribution using only MLP to generate scattered GPS points.
In addition, developing a tailor-made UNet architecture is also essential.
Comparing \cref{fig:diffunet} and \cref{fig:difftraj}, we can observe that the latter is able to generate a visually more realistic trajectory distribution.
This finding can be explained by the fact that Traj-UNet is capable of recording data features in a variety of domain-specific views and resolutions, which are essential for the entire diffusion process of Diff-Traj in \cref{sec:diffModel}.
% \note[02-02]{predicting the noise}{预测噪音听起来实在是奇怪，如果diffusion的人不刻意用这个词的话，全文都换一换。} in the \note[02-02]{reverse process}{哪个是reverse？你看，我读到这里都想不起来了，得给两三个词的准确指引。}.

Furthermore, we visualize the heat map of the trajectory distribution with multiple resolutions.
Specifically, we divide the whole city into $8\times8$, $16\times16$, and $32\times32$ grids, and then count the distribution of trajectories in each grid.
% \fix{Thanks to the excellent trajectory generation capability of Diff-Traj, the statistical results of all resolutions demonstrate the consistent spatial distribution pattern of trajectories within the city.}
The comparison clearly indicates that the distributions are highly consistent from all resolutions.
The visualized results also verify the effectiveness of metrics in \cref{tab:comp}, revealing that the proposed model can generate high-quality trajectories with remarkable accuracy and retain the original distribution.
% For those areas where the two distributions are slightly different, this is consistent with the basic fact of the density of trajectory distribution presented in \cref{fig:hetmap}
% \note[02-02]{}{这句话读起来有点怪，太空了，考虑重写。}
% \fix{While not obvious, the distribution is slightly different in concentrated areas, which is identical with the basic fact that regions with density human traffic are usually more complex for modeling.}{}

% Thanks to the excellent trajectory generation capability of Diff-Traj, the forged trajectory distribution is almost identical to the original case. This result is also consistent with the JS-Traj metrics from \cref{tab:comp}, which fully illustrates that the proposed model can generate high-quality trajectories with remarkable accuracy and retain the original distribution properties.






% 分布格子可视化  不同大小
% \subsection{Efficiency Evaluation}

% \begin{figure}[htbp]
%     \centering
%     \subfigure[Time steps $T$]{
%         \includegraphics[width=0.99\linewidth]{Figures/para_step.pdf}
%         \label{fig:paraS}
%     }
%     \quad 
%     \subfigure[Batch size $B$]{
%         \includegraphics[width=0.99\linewidth]{Figures/para_batchsize.pdf}
%         \label{fig:paraB}
%     }
%     \caption{Comparison of different parameters.}
%     \label{fig:para}
% \end{figure}



\subsection{Parameter Analysis}
When designing a diffusion model, how to set the optimal diffusion step size is a common question that needs to be answered for satisfactory generation performance.
In this section, we conduct experiments with Diff-Traj on two datasets to investigate the sensitivity of the diffusion process time steps $T$.
\cref{fig:paraS} shows the performance of $T\in\{50,100,200,300\}$, where we can observe that the parameter directly affects the generated results.
For ($T \leq 100$), Diff-Traj suffers from too small a diffusion process (i.e.,\cref{eq:qxtx0}), causing the trajectory generated by Diff-Traj concentrated in parts of the city.
The root cause is that the trajectories are non-iid within cities (c.f. \cref{fig:hetmap} in the \cref{app:dataset}).
A small diffusion $T$ causes the model to focus on the most important areas, ignoring the margins of the city.
On the other hand, with $T$ increases ($T\ge200$), the results generated by Diff-Traj are shown to cover most of the area throughout the city.
The results follow the widely recognized diffusion model principle that a sufficiently large diffusion step can improve its expressibility and thus utilize more significant potential features for data generation.
However, the large diffusion step leads to a long sampling time during generation, which makes the Diff-Traj computationally expensive and inefficient.
Therefore, Diff-Traj needs to integrate a method (presented in \cref{sec:ddim}) that guarantees the generation quality while speeding up the sampling.

% \note[02-02]{speeding up the sampling}{前文有介绍这个东西吗？是在实验部分新加的模块？}.\notemar[02-02]{这里前后开始，文法错误变得多了一些。把全文的大段文字部分，用quillbot或者chatgpt过一过吧。}

 
\begin{figure}[!t]
    \includegraphics[width=0.95\linewidth]{Figures/para_step.pdf}
    \caption{Comparison of different diffusion steps $T$.}
    \label{fig:paraS}
    % \vspace{-3mm}
\end{figure}


\begin{figure}[t]
    \centering
    \subfigure[Chengdu]{
        \includegraphics[width=0.45\linewidth]{Figures/steps_chengdu.pdf}
    }
    \subfigure[Xi'an]{
        \includegraphics[width=0.45\linewidth]{Figures/steps_xian.pdf}
    }
    % \vspace{-3mm}
    \caption{Sampling Efficiency Comparison.}
    \label{fig:ddim}
    % \vspace{-4mm}
\end{figure}

\subsection{Speed up Sampling}
As introduced in \cref{sec:method}, the diffusion model requires a considerable sampling step to gradually denoising for generation. 
This is also verified by results shown in \cref{fig:paraS}.
In actuality, it leads Diff-Traj to generate trajectories rather slowly.
Therefore, we integrate the speed-up sampling technique in Diff-Traj and examine its efficiency in this section.
Specifically, through incorporating sampling speed-up technique discussed in \cref{sec:ddim}, we generate $50 \times 256 $ trajectories based on a well-trained Diff-Traj on two datasets.

The results are summarized in \cref{fig:ddim}, where the two Y-axes represent the time spent and the JS-Traj score, respectively.
Here, the total sampling step is $T=300$ and the X-axis represents the sample steps after speed up, e.g., sampling every $6$ steps  if $S=50$.
We observe that all models trained with $T = 300$ diffusion steps unsurprisingly yield high-quality trajectories similar to the original distribution.
In the meantime, the model manages to match the outcomes of the no skipped steps method at $T = 50$ while saving $82\%$ of the time cost.
However, too few sampling steps ($S < 50$) lead to a substantial distribution divergence between the forged trajectories and real ones.
The reason is that with fewer sample steps, more reverse operations have to be skipped, rendering Diff-Traj discarding more noisy information during the denoising process.
Nevertheless, this result adequately indicates the outstanding contribution of the speeding up methods (in \cref{sec:ddim}) for efficiency improvement.
% \note[02-03]{integrated method}{指代不明} 
% \fix{Therefore, while employing the Diff-Traj for trajectory generation, we can appropriately skip the sample step to generate high-quality trajectories with fewer steps.}{}




% 事实上通过跳跃采样， 50步就能取得不错的结果，速度提升82%


% 50*256 条轨迹
% \begin{table}[!t]
% \caption{Sampling Efficiency Comparison.}
% \centering
% \begin{tabular}{ccccccc}
% \toprule
% \multicolumn{2}{c}{\multirow{2}{*}{City}} &    & \multicolumn{4}{c}{S} \\ \cmidrule(lr){3-7}

%                           &  & 10  & 30  & 50 & 300 \\
%  \cmidrule(lr){1-7}                         
% \multirow{2}{*}{Chengdu }        &time          & \SI{0.23}{\minute}    & \SI{1.10}{\minute}    & \SI{1.57}{\minute} & \SI{11.48}{\minute}  \\
% & JS-Traj      &  0.0157 &  0.0038   &  0.0029     & 0.0027    \\
%  \cmidrule(lr){1-7} 
% \multirow{2}{*}{Xi'an}  &time  & \SI{0.24}{\minute}    & \SI{1.09}{\minute}    & \SI{1.56}{\minute} &   \SI{11.52}{\minute} \\ 
% & JS-Traj      & 0.0218  &  0.0084   &  0.0054   &  0.0049   \\
% \bottomrule
% \end{tabular}
% \label{tab:eff}
% \end{table}







\subsection{Utility of Generated Data}
% \vspace{+8mm}
% Data utility is an essential criterion for trajectory generation. 
% In this section, we explore the utility through the map-matching task.
% Specifically, we evaluate the map-matching rate of the forged trajectory and visualize it according to the fast map-matching method proposed in \cite{fmm}.
% % 通过真实地图mmr和可视化来探究数据可用性
% As concluded in \cref{tab:comp}, the trajectories generated by Diff-Traj achieved higher MMR scores.
As the forged trajectories serve downstream tasks, their utility is critical to determine whether the data generation method is indeed practical.
In this section, we evaluate the utility of forged trajectories through map-matching, which is a common pre-processing technique in various applications \cite{zhu2022cross,ruan2020learning}.
Specifically, we evaluate the map-matching rate of the forged trajectories and visualize them according to the fast map-matching method \cite{fmm}.
As concluded in \cref{tab:comp}, trajectories generated by Diff-Traj achieved the best MMR scores, where the Chengdu dataset enjoys better results than Xi'an.
The result is aligned with the road conditions in both cities, i.e., the roads in the Xi'an dataset are shorter and more intensive, making it challenging to match the maps.
We further delve into a specific region and visualize the forged trajectories in \cref{fig:utility}, where the red dashed line indicates forged ones, and the blue dotted line indicates matched ones.
Compared to other results, trajectories from Diff-Traj are more aligned with the road network, which implies a higher utility.
Those compared methods may cause significant errors in map-matching and potentially undermine downstream service performance.
These findings are also confirmed by \cref{fig:resultcompchengdu}, where Diff-Traj holds a smaller offset from roads.


\begin{figure}[t]
    \centering
    \subfigure[VAE]{
        \includegraphics[width=0.46\linewidth]{Figures/case_traj_vae.pdf}
    }
    \subfigure[Traj-GAN]{
        \includegraphics[width=0.46\linewidth]{Figures/case_traj_gan.pdf}
    }
    \hfill
    \subfigure[Diff-wo/UNet]{
        \includegraphics[width=0.46\linewidth]{Figures/case_traj_mlp.pdf}
    }
    \subfigure[Diff-Traj]{
        \includegraphics[width=0.46\linewidth]{Figures/case_traj_ddpm.pdf}
    }
    % \vspace{-3mm}
    \caption{Forged trajectories map matching result (Red dashed line -- generated; blue line -- matched).}
    \label{fig:utility}
    % \vspace{-6mm}
\end{figure}

% \subsection{Data Utility}
% % 做一个简单的任务，ETA，用两三个模型对比一下
% % 不行就地图匹配或者别的
